Strong Reductions between Relatives of the Stable Ramsey's Theorem

A complete analysis is given of the computable reductions that hold between $\mathsf{SRT}^2_2$, $\mathsf{SPT}^2_2$, and $\mathsf{SIPT}^2_2$. In particular, while $\mathsf{D}^2_2\le_{\rm sW}\mathsf{SIPT}^2_2\le_{\rm sW}\mathsf{SPT}^2_2\le_{\rm sW}\mathsf{SRT}^2_2$, it is shown that $\mathsf{SRT}^2_2\not\le_{\rm sc}\mathsf{SPT}^2_2\not\le_{\rm sc}\mathsf{SIPT}^2_2\not\le_{\rm sc}\mathsf{D}^2_2$.

==> basicresults.tex <==
\begin{theorem}
$\mathsf{SIPT}^2_2\not\le_{\rm sc}\mathsf{D}^2_2$.
\end{theorem}

\textbf{Proof of Theorem.}
Let $f:[\omega]^2\to 2$ be an instance of $\mathsf{SIPT}^2_2$ all of whose solutions compute $\emptyset'$. Every instance of $\mathsf{D}^2_2$---in particular, every instance computable from $f$---has a solution which does not compute $\emptyset'$, hence does not compute any infinite set increasing $p$-homogeneous for $f$. \hfill $\blacksquare$


\begin{theorem}
$\mathsf{SRT}^2_2 \le_{\rm W} \mathsf{SPT}^2_2\le_W \mathsf{SIPT}^2_2$. 
\end{theorem}

\begin{lemma}
Fix $i<2$. There is a Turing functional $\Phi_i$ such that if $f:[\omega]^2\to 2$ is a stable 2-coloring of pairs and $L$ is an infinite set limit homogeneous for $f$ with color $i$, then $\Phi^{L\oplus\{i\}}$ describes an infinite set $H$ homogeneous for $f$. 
\end{lemma}

\textbf{Proof of Lemma.} Fix $f$ and $L$. We may compute from $L\oplus\{i\}$ an infinite set $H = \{h_0,h_1,h_2,\dots\}$ homogeneous for $f$ as follows. Let $h_0$ be the least element of $L$, $h_1$ the least element of $L$ such that $\{h_0,h_1\}$ is finite homogeneous for $f$, and $h_{k+1}$ the least element of $L$ such that $\{h_0,h_1,\dots,h_k\}$ is finite homogeneous for $f$. The stability of $f$ and the fact that $L$ is limit homogeneous for $f$ with color $i$ imply that this enumeration is computable; this together with the ordering of enumeration implies that $H$ is computable in the given data. \hfill $\blacksquare$ \\ 

\textbf{Proof of Theorem.} 

Fix a stable 2-coloring of pairs $f:[\omega]^2\to 2$ and an infinite set $I = I_0\oplus I_1$ increasing $p$-homogeneous for $f$. Let $i_0,i_1$ be the two least elements of $I_0$. Because $f$ is stable and $I$ is increasing $p$-homogeneous for $f$, $I_0$ is limit homogeneous for $f$ with color $f(i_0,i_1)$. Since $f(i_0,i_1)$ and $I_0$ are computable from $f\oplus I$, by the lemma $f\oplus I$ computes an infinite set $H$ homogeneous for $f$, hence the infinite set $H\oplus H$ $p$-homogeneous for $f$. \hfill $\blacksquare$
